pixelSplat: 3D Gaussian Splats from Image Pairs for Scalable Generalizable 3D Reconstruction

We introduce pixelSplat, a feed-forward model that learns to reconstruct 3D radiance fields parameterized by 3D Gaussian primitives from pairs of images. Our model features real-time and memory-efficient rendering for scalable training as well as fast 3D reconstruction at inference time. To overcome local minima inherent to sparse and locally supported representations, we predict a dense probability distribution over 3D and sample Gaussian means from that probability distribution. We make this sampling operation differentiable via a reparameterization trick, allowing us to back-propagate gradients through the Gaussian splatting representation. We benchmark our method on wide-baseline novel view synthesis on the real-world RealEstate10k and ACID datasets, where we outperform state-of-the-art light field transformers and accelerate rendering by 2.5 orders of magnitude while reconstructing an interpretable and editable 3D radiance field.

==> figs/comparison_acid/comparison_acid.tex <==
\begin{figure*}[t]
    \centering
    \def\svgwidth{\textwidth}
    \includesvg[width=1.067254\textwidth]{figs/comparison_acid/comparison_acid.svg}
    \vspace{-10pt}
    \caption{\textbf{Qualitative comparison of novel views on RealEstate10k (top) and ACID (bottom) test sets.} Compared to the baselines, our approach not only produces more accurate and perceptually more pleasing images, but also generalizes better to out-of-distribution examples like the creek on the bottom row.}
    \label{fig:comparison_acid}
    \vspace{-1em}
\end{figure*}


==> figs/comparison_re10k/comparison_re10k.tex <==
\begin{figure*}[t]
    \centering
    \def\svgwidth{\textwidth}
    \includesvg[width=1.067254\textwidth]{figs/comparison_re10k/comparison_re10k.svg}
    \vspace{-10pt}
    \label{fig:comparison_re10k}
    \vspace{-1em}
\end{figure*}


==> figs/epipolar_sampling/epipolar_sampling.tex <==
\begin{figure}[!t]
    \centering
    \includesvg[width=\linewidth]{figs/epipolar_sampling/epipolar_sampling.svg}
    \vspace{-15pt}
    \caption{\textbf{Epipolar sampling.} The ray on the left corresponds to the epipolar line on the right. Samples along this line are annotated with their depths. For a given ray, our epipolar cross-attention layer uses features from the ray's location (left panel) to attend to features sampled along the corresponding epipolar line (right panel), which are augmented with depth information. Our samples are drawn linearly in image space, resulting in non-linear depth increments between samples.}
    \label{fig:epipolar_sampling}
\end{figure}

